Whose doctor does the AI recommend? An algorithm audit of reputation and demographic signals in large language model-assisted physician choice

Patients increasingly ask large language model (LLM) assistants which doctor to see, making these systems AI infomediaries: algorithms that intermediate one person's choice among other people and thereby decide, silently and at scale, which physicians become visible. We report a prespecified randomized algorithm audit of what causally moves those recommendations. Seven models (six open-weight; gpt-4o-mini) each chose among five synthetic family-medicine physician cards whose attributes were independently randomized across 3,024 choice sets, three patient personas, nine prompt paraphrases and nine experimental arms, yielding 40,068 scored responses; gender and ethnicity were signaled through names following correspondence-audit methodology. Reputation signals dominate: raising a rating from 3.9 to 4.7 increases choice probability by 31.4 percentage points (pp), and raising the fee from $90 to $190 lowers it by 20.0 pp. Demographic parity is rejected, but not in the direction human audit studies predict: female-signaled names gain 2.5 pp, and Hispanic-, South-Asian- and Black-signaled names gain 1.3-2.9 pp over White-signaled names, tilts worth $7-$14 per visit in fee-equivalent terms, and a content-free first-listed position is worth $11. Yet models mentioned gender or ethnicity in at most 0.03% of their stated reasons and abstained in 0.39% of trials, so these effects are invisible in the models' own explanations, and transparency obligations relying on model self-report would not detect them. One reasoning model failed the prespecified auditability gate outright. The frozen design makes the audit repeatable: any new model can be assessed against identical stimuli, making recurring behavioural audit, rather than self-reported explanation, the monitoring technology fit for purpose.

==> sections/ai_declaration.tex <==
\section*{Declaration of generative AI use}
Large language models are the \emph{object of study} in this work: all model
outputs entering confirmatory analyses were collected under the prespecified
audit protocol described in Section~3. Separately, the authors used an AI
coding assistant (Claude, Anthropic) to help implement the experiment
pipeline and analysis code and to assist with drafting and editing the
manuscript under author direction. One dataset straddles these roles and is
disclosed accordingly: the exploratory frontier-model session pilot
(Section~3) was collected \emph{inside} the coding-assistant environment, so
the piloted Claude-family models, including the model family of the
assistant itself, responded within an agent harness rather than as bare API
calls; those records are quarantined from all confirmatory estimates and
reported only descriptively. All analyses, results, and claims were verified
by the authors, who take full responsibility for the content.


==> tables/tab_amce_main.tex <==
\begin{table}[t]
\centering
\caption{Average marginal component effects on P(recommended), pooled across the model panel (percentage points).}
\label{tab:amce_main}
\begin{tabular}{lrrr}
\toprule
Attribute & AMCE (pp) & 95\% CI & $P$ \\
\midrule
Rating 4.3 (vs 3.9) & 8.06 & [7.34, 8.78] & <.001 \\
Rating 4.7 (vs 3.9) & 31.38 & [30.48, 32.29] & <.001 \\
85 reviews (vs 12) & 4.79 & [3.93, 5.64] & <.001 \\
400 reviews (vs 12) & 8.44 & [7.56, 9.31] & <.001 \\
Recent review (vs 11 mo.) & 3.80 & [3.09, 4.51] & <.001 \\
Responds to patient feedback & 2.09 & [1.37, 2.80] & <.001 \\
Hospital-affiliated (vs independent) & 0.34 & [-0.37, 1.04] & .349 \\
\textbackslash\{\}\$140 fee (vs \textbackslash\{\}\$90) & -14.46 & [-15.45, -13.46] & <.001 \\
\textbackslash\{\}\$190 fee (vs \textbackslash\{\}\$90) & -20.02 & [-20.96, -19.08] & <.001 \\
Telehealth available & 2.78 & [2.08, 3.49] & <.001 \\
18 yrs in practice (vs 8) & 0.85 & [-0.01, 1.72] & .052 \\
28 yrs in practice (vs 8) & 2.08 & [1.21, 2.96] & <.001 \\
Female name (vs male) & 2.51 & [1.81, 3.20] & <.001 \\
Black name (vs White) & 1.33 & [0.25, 2.42] & .016 \\
Hispanic name (vs White) & 2.81 & [1.69, 3.93] & <.001 \\
East Asian name (vs White) & 0.25 & [-0.84, 1.34] & .653 \\
South Asian name (vs White) & 2.88 & [1.74, 4.01] & <.001 \\
Position 2 (vs 1) & 0.68 & [-0.54, 1.89] & .274 \\
Position 3 (vs 1) & -0.23 & [-1.42, 0.97] & .711 \\
Position 4 (vs 1) & -3.31 & [-4.48, -2.14] & <.001 \\
Position 5 (vs 1) & -6.15 & [-7.26, -5.04] & <.001 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/tab_confirmatory.tex <==
\begin{table}[t]
\centering
\caption{Confirmatory hypothesis tests (joint Wald tests, Holm-corrected).}
\label{tab:confirmatory}
\begin{tabular}{lrrrr}
\toprule
Hypothesis & Wald & df & $P$ (raw) & $P$ (Holm) \\
\midrule
H1\_rating & 4636.25 & 2 & <.001 & <.001*** \\
H2\_volume & 363.61 & 2 & <.001 & <.001*** \\
H3\_recency & 111.31 & 1 & <.001 & <.001*** \\
H4\_response & 32.42 & 1 & <.001 & <.001*** \\
H5\_network & 0.88 & 1 & .349 & .349 \\
H6\_price & 1745.92 & 2 & <.001 & <.001*** \\
H7\_telehealth & 59.80 & 1 & <.001 & <.001*** \\
H8\_experience & 22.08 & 2 & <.001 & <.001*** \\
H9\_gender & 49.90 & 1 & <.001 & <.001*** \\
H10\_ethnicity & 44.67 & 4 & <.001 & <.001*** \\
H11\_persona\_x\_price & 834.63 & 6 & <.001 & <.001*** \\
H12\_rating\_x\_volume & 170.90 & 4 & <.001 & <.001*** \\
H13\_intersectional & 9.51 & 4 & .050 & .099 \\
\bottomrule
\end{tabular}
\\[2pt]
{\footnotesize\textit{Note.} Holm-corrected over the H1--H12 confirmatory family. $^{*}p<.05$, $^{**}p<.01$, $^{***}p<.001$.}
\end{table}


==> tables/tab_importance.tex <==
\begin{table}[t]
\centering
\caption{Attribute importance: range of AMCEs and normalized share.}
\label{tab:importance}
\begin{tabular}{lrr}
\toprule
Attribute & Range (pp) & Share \\
\midrule
Patient rating & 31.38 & 0.377 \\
Visit fee & 20.02 & 0.241 \\
Review volume & 8.44 & 0.101 \\
List position & 6.83 & 0.082 \\
Recency & 3.80 & 0.046 \\
Ethnicity (name-signaled) & 2.88 & 0.035 \\
Telehealth & 2.78 & 0.033 \\
Gender (name-signaled) & 2.51 & 0.030 \\
Feedback response & 2.09 & 0.025 \\
Experience & 2.08 & 0.025 \\
Affiliation & 0.34 & 0.004 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/tab_intersectional.tex <==
\begin{table}[t]
\centering
\caption{Intersectional gender $\times$ ethnicity effects on P(recommended).}
\label{tab:intersectional}
\begin{tabular}{lrrrr}
\toprule
Gender $\times$ ethnicity cell & AMCE (pp) & 95\% CI & $P$ & TOST $P$ \\
\midrule
White male (ref.) & 0.00 & -- & -- & -- \\
Black male & 0.52 & [-1.02, 2.05] & .510 & .104 \\
Hispanic male & 1.74 & [0.19, 3.30] & .028 & .620 \\
East Asian male & 0.77 & [-0.79, 2.32] & .333 & .177 \\
South Asian male & 2.41 & [0.81, 4.01] & .003 & .868 \\
White female & 1.81 & [0.26, 3.35] & .022 & .651 \\
Black female & 3.93 & [2.39, 5.46] & <.001 & .999 \\
Hispanic female & 5.65 & [4.04, 7.27] & <.001 & 1.000 \\
East Asian female & 1.46 & [-0.06, 2.99] & .060 & .482 \\
South Asian female & 5.12 & [3.50, 6.74] & <.001 & 1.000 \\
\bottomrule
\end{tabular}
\\[2pt]
{\footnotesize\textit{Note.} Effect of each name-signaled cell vs.\ White male, from a single 10-level categorical (choice-set--clustered SEs). TOST $p<.05$ indicates statistical equivalence within $\pm$1.5 pp.}
\end{table}


==> tables/tab_letter.tex <==
\begin{table}[t]
\centering
\caption{Letter-arm decomposition of list-position effects from letter-token preferences (linear probability model on first-token letter probabilities, trial-clustered SEs).}
\label{tab:letter}
\begin{tabular}{lrrr}
\toprule
Term & Coef. (pp) & SE (pp) & $P$ \\
\midrule
Position 2 (vs 1) & 4.42 & 3.50 & .206 \\
Position 3 (vs 1) & 7.95 & 3.59 & .027 \\
Position 4 (vs 1) & 3.99 & 3.44 & .246 \\
Position 5 (vs 1) & 1.24 & 3.30 & .707 \\
Letter B (vs A) & 0.82 & 3.68 & .824 \\
Letter C (vs A) & 2.90 & 3.75 & .438 \\
Letter D (vs A) & -0.73 & 3.61 & .839 \\
Letter E (vs A) & -7.28 & 3.26 & .025 \\
\bottomrule
\end{tabular}
\\[2pt]
{\footnotesize\textit{Note.} Position block incremental $R^2$ = 0.0050; letter-token block = 0.0077. Slot and letter are independently randomized by design.}
\end{table}


==> tables/tab_parse.tex <==
\begin{table}[t]
\centering
\caption{Response parse-failure rates.}
\label{tab:parse}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrrrrr}
\toprule
Model & card\_reversed & field\_order & grounded & letter & main & nopersona & rank\_top3 & retest & temp0 \\
\midrule
gemma3:4b & 0.0 & 0.0 & 0.0 & 0.0 & 0.8 & 0.0 & 0.0 & 0.0 & 0.0 \\
gpt-4o-mini & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
llama3.1:8b & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
llama3.2:3b & 0.0 & 0.0 & 0.0 & 1.7 & 0.0 & 0.0 & 0.7 & 0.0 & 0.0 \\
mistral:7b-instruct-q4\_K\_M & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 14.1 & 32.0 & 0.0 \\
phi3:mini & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 7.1 & 0.0 & 0.0 \\
qwen2.5:3b & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
\bottomrule
\end{tabular}
}
\\[2pt]
{\footnotesize\textit{Note.} Parse-failure rate (\%) by model and arm; pilot and manipulation-check calls excluded.}
\end{table}


==> tables/tab_retest.tex <==
\begin{table}[t]
\centering
\caption{Test--retest consistency of recommendations.}
\label{tab:retest}
\begin{tabular}{lrr}
\toprule
Model & Modal share & Entropy \\
\midrule
gemma3:4b & 0.993 & 0.015 \\
gpt-4o-mini & 0.967 & 0.064 \\
llama3.1:8b & 0.919 & 0.155 \\
llama3.2:3b & 0.856 & 0.295 \\
mistral:7b-instruct-q4\_K\_M & 0.732 & 0.560 \\
phi3:mini & 0.822 & 0.368 \\
qwen2.5:3b & 0.865 & 0.274 \\
\bottomrule
\end{tabular}
\\[2pt]
{\footnotesize\textit{Note.} Mean over test--retest choice sets (5 repetitions each).}
\end{table}


==> tables/tab_tradeoffs.tex <==
\begin{table}[t]
\centering
\caption{Fee-equivalent trade-offs (\$/visit) with Krinsky--Robb 95\% CIs.}
\label{tab:tradeoffs}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
Attribute & Pooled & New in town & Chronic care & Budget \\
\midrule
Rating 4.3 (vs 3.9) & 40.3 [36.1, 44.6] & 85.2 [72.5, 100.4] & 93.0 [78.8, 110.0] & 14.2 [10.3, 18.1] \\
Rating 4.7 (vs 3.9) & 156.8 [147.4, 167.2] & 366.4 [321.9, 425.1] & 343.5 [301.3, 396.6] & 46.5 [42.1, 51.1] \\
85 reviews (vs 12) & 23.9 [19.4, 28.5] & 66.6 [52.4, 83.1] & 57.3 [43.3, 73.3] & 4.3 [0.4, 8.2] \\
400 reviews (vs 12) & 42.2 [37.2, 47.3] & 106.5 [89.4, 127.1] & 105.9 [89.0, 126.2] & 7.6 [3.6, 11.7] \\
Recent review (vs 11 mo.) & 19.0 [15.4, 22.7] & 42.6 [31.3, 55.6] & 41.8 [30.6, 54.2] & 6.8 [3.5, 10.0] \\
Responds to patient feedback & 10.4 [6.9, 14.1] & 13.7 [3.0, 25.1] & 22.3 [11.7, 33.0] & 5.7 [2.3, 9.1] \\
Hospital-affiliated (vs independent) & 1.7 [-1.8, 5.2] & 10.4 [0.0, 21.7] & 19.1 [8.5, 30.4] & -5.8 [-8.9, -2.7] \\
Telehealth available & 13.9 [10.3, 17.5] & 25.6 [14.9, 37.0] & 28.8 [18.8, 40.1] & 6.1 [2.9, 9.4] \\
18 yrs in practice (vs 8) & 4.3 [-0.1, 8.5] & 13.3 [0.4, 26.6] & 7.5 [-4.9, 20.3] & 2.8 [-1.0, 6.7] \\
28 yrs in practice (vs 8) & 10.4 [6.1, 14.9] & 21.0 [8.0, 34.9] & 31.3 [18.4, 45.0] & 3.1 [-0.9, 7.0] \\
Female name (vs male) & 12.5 [9.0, 16.0] & 31.4 [20.9, 43.3] & 28.0 [18.0, 39.2] & 2.4 [-0.8, 5.6] \\
Black name (vs White) & 6.7 [1.3, 12.2] & 5.0 [-11.0, 21.3] & 18.7 [3.0, 35.4] & 5.4 [0.5, 10.4] \\
Hispanic name (vs White) & 14.1 [8.4, 19.8] & 28.6 [12.3, 46.0] & 17.4 [1.0, 34.7] & 8.9 [3.5, 14.1] \\
East Asian name (vs White) & 1.2 [-4.3, 6.8] & -0.2 [-15.7, 15.2] & 2.8 [-12.5, 18.6] & 1.0 [-4.3, 6.1] \\
South Asian name (vs White) & 14.3 [8.7, 20.3] & 23.3 [6.6, 40.6] & 23.2 [6.7, 40.9] & 8.3 [3.0, 13.6] \\
First-listed (vs avg 2-5) & 11.3 [6.5, 16.0] & 39.3 [24.9, 55.0] & 19.9 [7.0, 33.3] & 0.0 [-3.7, 3.7] \\
\bottomrule
\end{tabular}
}
\end{table}

